Neural Contraction Metrics with Formal Guarantees for Discrete-Time Nonlinear Dynamical Systems

Contraction metrics are crucial in control theory because they provide a powerful framework for analyzing stability, robustness, and convergence of various dynamical systems. However, identifying these metrics for complex nonlinear systems remains an open challenge due to the lack of scalable and effective tools. This paper explores the approach of learning verifiable contraction metrics parametrized as neural networks (NNs) for discrete-time nonlinear dynamical systems. While prior works on formal verification of contraction metrics for general nonlinear systems have focused on convex optimization methods (e.g. linear matrix inequalities, etc) under the assumption of continuously differentiable dynamics, the growing prevalence of NN-based controllers, often utilizing ReLU activations, introduces challenges due to the non-smooth nature of the resulting closed-loop dynamics. To bridge this gap, we establish a new sufficient condition for establishing formal neural contraction metrics for general discrete-time nonlinear systems assuming only the continuity of the dynamics. We show that from a computational perspective, our sufficient condition can be efficiently verified using the state-of-the-art neural network verifier $\alpha,\!\beta$-CROWN, which scales up non-convex neural network verification via novel integration of symbolic linear bound propagation and branch-and-bound. Built upon our analysis tool, we further develop a learning method for synthesizing neural contraction metrics from sampled data. Finally, our approach is validated through the successful synthesis and verification of NN contraction metrics for various nonlinear examples.

==> sections/complicated_main_theory.tex <==
\begin{theorem}\label{thm:main}
    Assume that $\mathcal{X}$ is an open, connected, and forward invariant subset in $\mathbb{R}^n$, and the dynamics function $f$ is continuous. Given $\epsilon > 0$ a small positive threshold. Suppose there exists continuous $M(x) : \mathcal{X} \to \mathbb{S}^{n\times n}_{++}$ with a uniform lower bound $M(x) \geq \mu I$ and 
    \begin{align}\label{verification}
         \sqrt{(f(x) - f(y))^TM(f(x))(f(x)-f(y))} \leq \rho \sqrt{(x-y)^TM(x)(x-y)} 
    \end{align}
    for all $x \in \mathcal{X}$ and $y \in \mathcal{B}_\epsilon(x) \cap \mathcal{X}$ and some $0< \rho < 1$. We denote $\lambda_n$ to be the Lebesgue measure on $\mathbb{R}^n$ and we further assume that the set of non-differentiable points $G$ of the dynamics $f$ has measure zero under $\lambda_n$. We denote the set of continuous piecewise smooth curves that avoid the non differentiable points of $f$ as
    \begin{align}
        \Gamma_{x,y}^f := \{\gamma : [0,1] \to \mathcal{X}, \text{$\gamma$ piecewise $C_\infty$}, \lambda_1(\{t: \gamma(t) \in G\}) = 0, \gamma(0) = x, \gamma(1) = y\}.
    \end{align}
     It is then guaranteed that the system~\eqref{eq:system} is contracting on $\mathcal{X}$ in the metric
    \begin{align}\label{metric}
        d(x,y) &= \inf_{\gamma \in \Gamma_{x,y}^f} \int \sqrt{\gamma'(t)^T M(\gamma(t))\gamma'(t)} \, d\lambda_1|_{[0,1]}
    \end{align}
    where the integration is with respect to the restriction of $\lambda_1$ on the interval $[0,1]$. 
\end{theorem} 

\begin{lemma}
    The defined metric $d: \mathbb{R}^n \times \mathbb{R}^n \to \mathbb{R}$ in~\eqref{metric} is a valid metric. 
\end{lemma}
\textbf{Proof:} Before demonstrating the three metric properties of 
$d$, we first verify that $d$ is well-defined. To begin, we show that $\Gamma_{x,y} \neq \emptyset$ for any $x,y \in \mathcal{X}$. Since by assumption $\mathcal{X}$ is a open and connected subset of $\mathbb{R}^n$, it is path-connected. Therefore, there exists a continuous curve $\gamma:[0,1] \to \mathcal{X}$ such that $\gamma(0) =x$ and $\gamma(1) = y$. If $n = 1$, $\mathcal{X}$ by assumption must be an open interval, and the straight line $\gamma(t) = x + (y-x)t$ clearly belongs to $\Gamma_{x,y}$. Therefore, we assume that $n > 1$ in the following analysis. It is well-known the existence of a continuous curve implies the existence of a piecewise smooth curve for an open set in $\mathbb{R}^n$, so without loss of generality we can assume that the $\gamma$ above is piecewise smooth. We also assume that the velocity is nonzero almost everywhere, which is always possible by reparametrization. Now we construct a tube around this piecewise smooth curve that completely lies in $\mathcal{X}$. Formally, for points where this curve is differentiable, we compute its tangent vector $T(t) = \frac{\gamma'(t)}{||\gamma'(t)||}$, and then construct the $n-1$ normal vectors $N_1(t), \cdots, N_{n-1}(t)$ such that together with $T(t)$ they form an orthonormal basis of $\mathbb{R}^n$, moreover, we construct them in such a way that $N_i$ varies smoothly with $t$ almost everywhere. We define a function $\Phi: [0,1] \times \mathbb{R}^{n-1} \to \mathbb{R}^n$
\begin{align}
    \Phi(t,v) &= \gamma(t) + \sum_i v_i N_i(t)
\end{align}
A tube is then defined to be
\begin{align}
    U &= \{\Phi(t,v):t \in [0,1], ||v|| < \delta\}
\end{align}
for some $\delta$. And we shall show that there exists $\delta > 0$ such that $U \subset \mathcal{X}$. To do that, we notice that since $\mathcal{X}$ is open, for each $t \in [0,1]$, there exists an $\epsilon_i$ such that $B_{\epsilon_t}(\gamma(t)) \subset \mathcal{X}$. Now since $B_{\frac{\epsilon_t}{2}}(\gamma(t))$ is an open cover of $\gamma([0,1])$, there is a finite subcover $\{B_{\frac{\epsilon_{t_i}}{2}}(\gamma(t_i))\}_{i=1}^k$. Now we pick $\delta < \min(\frac{\epsilon_{t_i}}{2})$. For each $\gamma(t)$, there exists an $i$ such that $\gamma(t) \in B_{\frac{\epsilon_{t_i}}{2}}(\gamma(t_i))$. By triangle inequality,
\begin{equation}
\begin{aligned}
    ||\Phi(t,v) - \gamma(t_i)|| &\leq ||\Phi(t,v) - \gamma(t)|| + ||\gamma(t) - \gamma(t_i)||  \\& \leq ||\sum_i v_i N_i(t)|| + \frac{\epsilon_{t_i}}{2} \\
    &\leq \delta + \frac{\epsilon_{t_i}}{2} \leq \epsilon_{t_i}
\end{aligned}
\end{equation}
So by construction we have $\Phi(t,x) \in B_{\epsilon_{t_i}}(\gamma(t_i)) \subset \mathcal{X}$. Now with this tube constructed, we can construct a family of curves connecting $x$ and $y$ such that they fill up a space with positive measure. We consider the function $\eta(t) = \sin^2(\pi t)$ and consider the function
\begin{align}
    \gamma_v(t) &= \gamma(t) + \eta(t)\sum_i v_iN_i(t)
\end{align}
still with the constraint $||v||<\delta$. Note that this function defines a piecewise smooth curve for any $v$ since clearly all of $\gamma(t), \eta(t), N_i(t)$ are. Moreover, we have
\begin{align}
    \gamma_v(0) &= \gamma(0) + \eta(0)\sum_i v_iN_i(0) = x\\
    \gamma_v(1) &= \gamma(1) + \eta(1)\sum_i v_iN_i(1) = y
\end{align}
Finally, as $|\eta(t)| < 1$, it is clear that $\gamma_v(t)$ will be contained in the tube $U$, which then lies in the full domain $\mathcal{X}$. By construction $\gamma_v(t)$ defines a family of curves that occupies a subset of the tube $U$, and now we treat it as a function whose domain is $\{||v|| < \delta\} \times [0,1]$ and consider its Jacobian $J(v,t)$. We can compute it as
\begin{align}
    J(v,t) = [\eta(t)N_1(t), \cdots, \eta(t)N_{n-1}(t), \gamma'(t) + \eta'(t)\sum_i v_i N'_i(t)]
\end{align}
Therefore, when $v = 0$, the Jacobian is clearly independent and has nonzero determinant for alsmost every $t$ just by construction of $N_i(t)$. And since the matrix varies continuously with respect to $v$, there exists a $\delta' > 0$ such that $J(v,t)$ is invertible for all $||v|| < \delta$ and for almost every $t$. Now we take $\delta_b = \min(\delta, \delta')$ and compute the Lebesgue integral of the indicator function of the null set $G$ over the image $S$ of the function  $\gamma_v(t)$ with domain $\{v: ||v|| < \delta_b\} \times [0,1]$. The integral will evaluate to $0$ since $G$ has measure $0$. However, we could compute the same integral by pulling back the integral to the input domain by a change of variable, and we apply Fubini's theorem to get
\begin{align}
    0 &= \int_S 1_{G} \, d\lambda_n \\
     &= \int_{||v|| < \delta_b} \int_0^1 1_G(\gamma_v(t)) |J(v,t)|\, dt\, d\lambda_{n-1}
\end{align}
where $J$ is the Jacobian matrix. Therefore, we see that the inner integral vanishes for almost every $v$. And when this integral equals to $0$, we know that the inner term $1_G(\gamma_v(t)) |J(v,t)|$ vanishes for almost $t$. And since we construct the domain so that $|J(v,t)| > 0$ almost everywhere, we know that $1_G(\gamma_v(t)) = 0$` for almost every $t$. This implies that for almost every $v$ the curve $\gamma_v$ avoids the measure zero set $G$ for almost every $t$. More specifically, $\Gamma_{x,y}^f \neq \emptyset$. The metric is thus well-defined by the completeness of $\mathbb{R}$.

Now we are ready to show the three metric properties. First we show positivity. Clearly, since the integrand $\sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)}$ is positive almost everywhere as $M(\gamma(t)) \in \mathbb{S}_{++}^{n\times n}$, we have that $d(x,y) \geq 0$. And we can see that $d(x,x) = 0$ since the constant curve $\gamma(t) = x$ belongs to the class $\Gamma^f_{x,y}$ no matter $x \in G$ or not. Therefore, we have that
\begin{align}
    0 \leq d(x,x) \leq \int_0^1 \sqrt{0M(x)0} d\lambda_1 = 0
\end{align}
Moreover, we see that
\begin{equation}
\begin{aligned}
    d(x,y) &= \inf_{\gamma\in \Gamma^f_{x,y}} \int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, d\lambda_1 \\ &\geq \inf_{\gamma \in \Gamma_{x,y}} \int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, d\lambda_1 \\ &\geq \sqrt{\epsilon}\inf_{\gamma\in \Gamma_{x,y}} \int_{0}^1 ||\gamma'(t)|| \, d\lambda_1 \geq \sqrt{\epsilon}||x-y||
\end{aligned}
\end{equation}
where $\Gamma_{x,y}$ is the same as $\Gamma_{x,y}^f$ except that the condition that the curve has to avoid the measure zero set is removed. From this inequality, we see that $d(x,y) > 0$ for $x \neq y$. Next we show the symmetry. For any $\gamma \in \Gamma_{x,y}^f$, it is clear that the reverse curve $\tilde{\gamma}(t):= \gamma(1-t)$ is an element of $\Gamma_{y,x}^f$. By a change of variable we have
\begin{equation}
    \begin{aligned}
        \int_0^1 \sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)} \, dt &=  \int_0^1 \sqrt{\tilde{\gamma}(t)^TM(\tilde{\gamma}(t))\tilde{\gamma}'(t)} \, dt
    \end{aligned}
\end{equation}
So as the action of taking reverse curve gives a bijection between $\Gamma^f_{x,y}$ and $\Gamma^f_{y,x}$, we must have $d(x,y) = d(y,x)$. Finally we show triangle inequality. For any $\gamma_1 \in \Gamma_{x,y}^f$ and $\gamma_2 \in \Gamma_{y,z}^f$, we concat $\gamma_1$ and $\gamma_2$ to build $\gamma_3$
\begin{align}
    \gamma_3(t) = \begin{cases}
        \gamma_1(2t), \quad t \in [0,\frac{1}{2}] \\
        \gamma_2(2t - 1), \quad t \in [\frac{1}{2}, 1]
    \end{cases}
\end{align}
Clearly $\gamma_3$ is still piecewise smooth. And since we have $G_{\gamma_3} \subset G_{\gamma_1} \cup G_{\gamma_2}$ where $G_\gamma := \{t: \gamma(t) \in G\}$, clearly we have $\lambda_1(G_{\gamma_3}) = 0$ and therefore $\gamma_3 \in \Gamma_{x,z}^f$. Now by simple change of variable we have
\begin{equation}
    \begin{aligned}
        \int_{0}^1 \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt &= \int_{0}^1 \sqrt{\gamma_1'(t)^TM(\gamma_1(t))\gamma_1'(t)} \, dt + \int_{0}^1 \sqrt{\gamma_2'(t)^TM(\gamma_2(t))\gamma_2'(t)} \, dt
    \end{aligned}
\end{equation}
Now taking infimum over both side we will get $d(x,z) \leq d(x,y) + d(y,z)$. \hfill $\square$

\medskip
\noindent
\textbf{Proof of Thm~\ref{thm:main}} Now we are finally ready to show the implication from condition~\eqref{verification} to contraction under the metric~\eqref{metric}. Fix an $\rho' \in (\rho,1)$. For any $\gamma \in \Gamma_{x,y}^f$, we consider the curve $f(\gamma)$. As $\mathcal{X}$ is forward invariant, $f(\gamma)$ also belongs to $\mathcal{X}$. By the verification condition~\eqref{verification}, we know that for $\delta_t$ small enough we always have 
\begin{equation}\label{condition1}
\begin{aligned}
    (f(\gamma(t+\delta_t)) &- f(\gamma(t)))^TM(f(\gamma(t+\delta_t)))(f(\gamma(t+\delta_t)) - f(\gamma(t))) \\ &\leq \rho^2 (\gamma(t+\delta_t)-\gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t)-\gamma(t))\\
    &< \rho'^2 (\gamma(t+\delta_t)-\gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t)-\gamma(t))
\end{aligned}
\end{equation}
Now fix an $\epsilon > 0$, we know that $f(\gamma)$ is a continuous curve, so that we can construct a piecewise smooth curve $\gamma_p$ such that $||f(\gamma(t)) - \gamma_p(t)|| \leq \epsilon$ for any $t$. And by previous construction, we know that there exists $\delta > 0$ such that for any $||v|| < \delta$, almost all the piecewise smooth curve
\begin{align}
    \gamma_v(t) = \gamma_p(t) + \eta(t)\sum_{i}v_iN_i(t)
\end{align}
intersect $G$ only on a measure zero set with $N_i$ constructed using $\gamma_p$. Pick one specific such $\gamma_v$ now, and we would have 
\begin{align}
    ||\gamma_v(t) - \gamma_p(t)|| \leq \delta|\eta(t)| \leq \delta
\end{align}
Now suppose that we pick $\delta$ small enough such that $\delta < \epsilon$. By triangle inequality, we have
\begin{align}
    ||\gamma_v(t) - f(\gamma(t))|| \leq ||\gamma_v(t) - \gamma_p(t)|| + ||\gamma_p(t) - f(\gamma(t))|| \leq 2\epsilon
\end{align}
for any $t$. Now we see that we have
\begin{equation}
\begin{aligned}
    % |f(\gamma(t+\delta_t)) - f(\gamma(t))| &= f(\gamma(t+\delta_t)) - \gamma_v(t+\delta_t) + \gamma_v(t+\delta_t) - \gamma_v(t) + \gamma_v(t) -  f(\gamma(t)) \\ &\leq 4\epsilon + |\gamma_v(t + \delta_t) - \gamma_v(t)| \\
     |(f(\gamma(t+\delta_t)) - f(\gamma(t))) &- (\gamma_v(t+\delta_t) - \gamma_v(t))| \\ &\leq |f(\gamma(t+\delta_t)) - \gamma_v(t+\delta_t)| + |f(\gamma(t)) - \gamma_v(t)| \leq 4\epsilon
\end{aligned}
\end{equation}
Now by~\ref{condition1}, the inequality is strict when the contraction factor is $\rho'$. This gives us room to wiggle the curve $f(\gamma)$ to be $\gamma_v$, which clearly belongs to the set $\Gamma_{f(x),f(y)}^f$, when $\epsilon$ is chosen to be small enough as everything is continuous, and we shall still have the inequality
\begin{align}
    (\gamma_v(t+\delta_t) - \gamma_v(t))^TM(\gamma_v(t+\delta_t)))(\gamma_v(t+\delta_t) - \gamma_v(t)) \\ \leq \rho'^2(\gamma(t+\delta_t) - \gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t) - \gamma(t))
\end{align}
Now divide both side by $\delta_t^2$ and let it goes to zero, we get
\begin{align}
    \gamma_v'(t)^TM(\gamma_v(t))\gamma_v'(t) \leq \rho'^2\gamma'(t)^TM(\gamma(t))\gamma'(t)
\end{align}
almost everywhere except on those points where $\gamma$ or $\gamma_v$ are not differentiable. This then implies 
\begin{align}
    d(f(x),f(y)) &\leq \int_0^1 \sqrt{\gamma_v'(t)^TM(\gamma_v(t))\gamma_v'(t)} \, dt \\
    &\leq \rho'\int_0^1 \sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)} \, dt
\end{align}
Now taking infimum over $\gamma$ on the right hand side gives the desired contraction result.

\medskip
\noindent
The proof of $d(x,y)$ is indeed a metric is already well-known in the literature. \textcolor{blue}{ John Lee, Introduction to Smooth Manifold, pp 337.} But for completeness, we still provide a short proof. By the connectedness assumption, there exists a continuous curve connecting any $x,y \in \mathcal{X}$. So by the previous lemma, there exists a piecewise smooth curve connecting $x,y$, and thus $\Gamma_{x,y} \neq \emptyset$. Moreover, since the infimum is taken in $\mathbb{R}$, this quantity is always well-defined by the completeness of $\mathbb{R}$. Now we discussed the three metric properties. Clearly, since the integrand is positive almost everywhere as $M(\gamma(t)) \in \mathbb{S}_{++}^{n\times n}$, we have that $d(x,y) \geq 0$. And we can see that $d(x,x) = 0$ since the constant curve $\gamma(t) = x$ belongs to the class $\Gamma_{x,y}$.
Moreover, we see that
\begin{equation}
\begin{aligned}
    d(x,y) &= \inf_{\gamma \in \Gamma_{x,y}} \int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, d\lambda_1 \geq \sqrt{\mu}||x-y||
\end{aligned}
\end{equation}
From this inequality, we see that $d(x,y) > 0$ for $x \neq y$. Next we show the symmetry. For any $\gamma \in \Gamma_{x,y}$, it is clear that the reverse curve $\tilde{\gamma}(t):= \gamma(1-t)$ is an element of $\Gamma_{y,x}$. By a change of variable we have
\begin{equation}
    \begin{aligned}
        \int_0^1 \sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)} \, dt &=  \int_0^1 \sqrt{\tilde{\gamma}(t)^TM(\tilde{\gamma}(t))\tilde{\gamma}'(t)} \, dt
    \end{aligned}
\end{equation}
So as the action of taking reverse curve gives a bijection between $\Gamma_{x,y}$ and $\Gamma_{y,x}$, we must have $d(x,y) = d(y,x)$. Finally we show triangle inequality. For any $\gamma_1 \in \Gamma_{x,y}^f$ and $\gamma_2 \in \Gamma_{y,z}^f$, we concat $\gamma_1$ and $\gamma_2$ to build $\gamma_3$
\begin{align}
    \gamma_3(t) = \begin{cases}
        \gamma_1(2t), \quad t \in [0,\frac{1}{2}] \\
        \gamma_2(2t - 1), \quad t \in [\frac{1}{2}, 1]
    \end{cases}
\end{align}
Clearly $\gamma_3$ is still piecewise smooth. Now by simple change of variable we have
\begin{equation}
    \begin{aligned}
        \int_{0}^1 \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt &= \int_{0}^1 \sqrt{\gamma_1'(t)^TM(\gamma_1(t))\gamma_1'(t)} \, dt + \int_{0}^1 \sqrt{\gamma_2'(t)^TM(\gamma_2(t))\gamma_2'(t)} \, dt
    \end{aligned}
\end{equation}
Now taking infimum over both side we will get $d(x,z) \leq d(x,y) + d(y,z)$. 






==> sections/prelim.tex <==
This paper focused on the the idea of incremental stability and contraction metrics, which both provide a description to the asymptotic property of the differences between two solutions to the system. The formal definition goes as follows.


\begin{definition}
    [Contraction]
    The system~\eqref{eq:system} is said to be \textbf{contracting} on a forward invariant set $\mathcal{X} \in \mathbb{R}^n$ if there exists a metric $d: \mathbb{R}^n \to \mathbb{R}$ and a scalar $0 < \rho < 1$ such that
    \begin{align}\label{def:contraction}
        d(f(x), f(y)) \leq \rho d(x,y), \forall x, y \in \mathcal{X}
    \end{align}
    We call $d$ the corresponding contraction metric and $\rho$ the contraction rate.
\end{definition}

\begin{definition}
    [Incremental Stability]
    The system~\eqref{eq:system} is said to be \textbf{incrementally stable} with respect to some metric $d$ on a forward invariant set $\mathcal{X} \in \mathbb{R}^n$ if for any two initial points $x_0, x_0'$ we have
    \begin{align}
        \lim_{t\to\infty} d(\phi(t, x_0), \phi(t, x_0')) = 0,
    \end{align}
    i.e the distance measured using the metric $d$ between the two solution trajectory converges to $0$. Moreover, if we have
    \begin{align}
        d(\phi(t, x_0), \phi(t, x_0')) \leq \kappa d(x_0, x_0') \lambda^{-t}
    \end{align}
    for some $\kappa, \lambda$ such that $\kappa \lambda < 1$, the system is said to be \textbf{exponentially incrementally stable}.
\end{definition}

\noindent
The concept of a contraction map is closely related to the concept of incremental stability, in the sense that the concept of contracting with respect to the metric $d$ is equivalent to the exponential incremental stability with respect to the metric $d$. This is formalized in the below theorem.

% \noindent
% The metrics $d$ can be very complex, which poses challenge in how to find it in practice. In this paper, we propose a simple condition that guarantees the existence of a Riemannian type metric in which that can make sure the system is contracting.

% \begin{theorem}\label{thm:main}
%     Assume that $\mathcal{X}$ is an open, connected, and forward invariant subset in $\mathbb{R}^n$. Given $\epsilon > 0$ a small positive threshold. Suppose there exists continuous $M(x) : \mathcal{X} \to \mathbb{S}^{n\times n}_{++}$ with a uniform lower bound $M(x) \geq \mu I$ and 
%     \begin{align}\label{verification}
%          \sqrt{(f(x) - f(y))^TM(f(x))(f(x)-f(y))} \leq \rho \sqrt{(x-y)^TM(x)(x-y)} 
%     \end{align}
%     for all $x \in \mathcal{X}$ and $y \in \mathcal{B}_\epsilon(x) \cap \mathcal{X}$ and some $0< \rho < 1$. Denote $\lambda_n$ to be the Lebesgue measure on $\mathbb{R}^n$ and we further assume that the set of non-differentiable points $G$ of the dynamics $f$ has measure zero under $\lambda_n$. We denote the set of continuous piecewise smooth curves that avoid the non differentiable points of $f$ as
%     \begin{align}
%         \Gamma_{x,y}^f := \{\gamma : [0,1] \to \mathcal{X}, \text{$\gamma$ piecewise $C_\infty$}, \lambda_1(\{t: \gamma(t) \in G\}) = 0, \gamma(0) = x, \gamma(1) = y\}.
%     \end{align}
%      It is then guaranteed that the system~\eqref{eq:system} is contracting on $\mathcal{X}$ in the metric
%     \begin{align}\label{metric}
%         d(x,y) &= \inf_{\gamma \in \Gamma_{x,y}^f} \int \sqrt{\gamma'(t)^T M(\gamma(t))\gamma'(t)} \, d\lambda_1|_{[0,1]}
%     \end{align}
%     where the integration is with respect to the restriction of $\lambda_1$ on the interval $[0,1]$. 
% \end{theorem} 

% \begin{lemma}
%     The defined metric $d: \mathbb{R}^n \times \mathbb{R}^n \to \mathbb{R}$ in~\eqref{metric} is a valid metric. 
% \end{lemma}
% \textbf{Proof:} Before demonstrating the three metric properties of 
% $d$, we first verify that $d$ is well-defined. To begin, we show that $\Gamma_{x,y} \neq \emptyset$ for any $x,y \in \mathcal{X}$. Since by assumption $\mathcal{X}$ is a open and connected subset of $\mathbb{R}^n$, it is path-connected. Therefore, there exists a continuous curve $\gamma:[0,1] \to \mathcal{X}$ such that $\gamma(0) =x$ and $\gamma(1) = y$. If $n = 1$, $\mathcal{X}$ by assumption must be an open interval, and the straight line $\gamma(t) = x + (y-x)t$ clearly belongs to $\Gamma_{x,y}$. Therefore, we assume that $n > 1$ in the following analysis. It is well-known the existence of a continuous curve implies the existence of a piecewise smooth curve for an open set in $\mathbb{R}^n$, so without loss of generality we can assume that the $\gamma$ above is piecewise smooth. Also since we can do reparametrization by arc length, we also assume that the velocity is always nonzero. Now we construct a tube around this piecewise smooth curve that completely lies in $\mathcal{X}$. Formally, for points where this curve is differentiable, we compute its tangent vector $T(t) = \frac{\gamma'(t)}{||\gamma'(t)||}$, and then construct the $n-1$ normal vectors $N_1(t), \cdots, N_{n-1}(t)$ such that together with $T(t)$ they form an orthonormal basis of $\mathbb{R}^n$, moreover, we construct them in such a way that $N_i$ varies smoothly with $t$ almost everywhere. We define a function $\Phi: [0,1] \times \mathbb{R}^{n-1} \to \mathbb{R}^n$
% \begin{align}
%     \Phi(t,v) &= \gamma(t) + \sum_i v_i N_i(t)
% \end{align}
% A tube is then defined to be
% \begin{align}
%     U &= \{\Phi(t,v):t \in [0,1], ||v|| < \delta\}
% \end{align}
% for some $\delta$. And we shall show that there exists $\delta > 0$ such that $U \subset \mathcal{X}$. To do that, we notice that since $\mathcal{X}$ is open, for each $t \in [0,1]$, there exists an $\epsilon_i$ such that $B_{\epsilon_t}(\gamma(t)) \subset \mathcal{X}$. Now since $B_{\frac{\epsilon_t}{2}}(\gamma(t))$ is an open cover of $\gamma([0,1])$, there is a finite subcover $\{B_{\frac{\epsilon_{t_i}}{2}}(\gamma(t_i))\}_{i=1}^k$. Now if we pick $\delta < \min(\frac{\epsilon_{t_i}}{2})$, we can check that for the neighborhood such that $\gamma(t) \in B_{\frac{\epsilon_{t_i}}{2}}(\gamma(t_i))$
% \begin{equation}
% \begin{aligned}
%     ||\Phi(t,v) - \gamma(t_i)|| &\leq ||\Phi(t,v) - \gamma(t)|| + ||\gamma(t) - \gamma(t_i)||  \\& \leq ||\sum_i v_i N_i(t)|| + \frac{\epsilon_{t_i}}{2} \\
%     &\leq \delta + \frac{\epsilon_{t_i}}{2} \leq \epsilon_{t_i}
% \end{aligned}
% \end{equation}
% Now with this tube constructed, we can construct a family of curves connecting $x$ and $y$ such that they fill up a space with positive measure. We consider the function $\eta(t) = \sin^2(\pi t)$ and consider the function
% \begin{align}
%     \gamma_v(t) &= \gamma(t) + \eta(t)\sum_i v_iN_i(t)
% \end{align}
% still with the constraint $||v||<\delta$. Note that this function defines a piecewise smooth curve for any $v$ since clearly all of $\gamma(t), \eta(t), N_i(t)$ are. Moreover, we have
% \begin{align}
%     \gamma_v(0) &= \gamma(0) + \eta(0)\sum_i v_iN_i(0) = x\\
%     \gamma_v(1) &= \gamma(1) + \eta(1)\sum_i v_iN_i(1) = y
% \end{align}
% Finally, as $|\eta(t)| < 1$, it is clear that $\gamma_v(t)$ will be contained in the tube $U$, which then lies in the full domain $\mathcal{X}$. By construction $\gamma_v(t)$ defines a family of curves that occupies a subset of the tube $U$, and now we treat it as a function whose domain is $\{||v|| < \delta\} \times [0,1]$ and consider its Jacobian $J(v,t)$. We can compute it as
% \begin{align}
%     J(v,t) = [\eta(t)N_1(t), \cdots, \eta(t)N_{n-1}(t), \gamma'(t) + \eta'(t)\sum_i v_i N'_i(t)]
% \end{align}
% Therefore, when $v = 0$, the Jacobian is clearly independent and has positive determinant just by construction of $N_i(t)$. And since the matrix varies continuously with respect to $v$, there exists a $\delta' > 0$ such that $J(v,t)$ is invertible for all $||v|| < \delta$. Now we take $\delta_b = \min(\delta, \delta')$ Now we can compute the Lebesgue integral of the indicator function of the null set $G$ over the domain $\{v: ||v|| < \delta_b\} \times [0,1]$. The integral will evaluate to $0$ since $G$ has measure $0$. However, we could pullback the integral to the input domain rewrite the integral with Fubini's theorem and get
% \begin{align}
%     0 &= \int_S 1_{G} \, d\mu \\
%      &= \int_{||v|| < \delta_b} \int_0^1 1_G(\gamma_v(t)) |J(v,t)|\, dt\, d\lambda^{n-1}
% \end{align}
% where $J$ is the Jacobian matrix. Therefore, we see that the inner integral vanishes for almost every $v$. And when this integral equals to $0$, we know that the inner term $1_G(\gamma_v(t)) |J(v,t)|$ vanishes for almost $t$. And since we construct the domain so that $|J(v,t)| > 0$ almost everywhere except possibly on the points where $\gamma$ is non-differentiable, we know that $1_G(\gamma_v(t)) = 0$ for almost every $t$. This implies that for almost every $v$ we have for almost every $t$ that the curve $\gamma_v(t)$ avoids the measure zero set $G$. More specifically, $\Gamma_{x,y}^f \neq \emptyset$. The metric is thus well-defined by the completeness of $\mathbb{R}$.

% Now we are ready to show the three metric properties. First we show positivity. Clearly, since the integrand $\sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)}$ is positive almost everywhere as $M(\gamma(t)) \in \mathbb{S}_{++}^{n\times n}$, we have that $d(x,y) \geq 0$. And we can see that $d(x,x) = 0$ since the constant curve $\gamma(t) = x$ belongs to the class $\Gamma^f_{x,y}$ no matter $x \in G$ or not. Therefore, we have that
% \begin{align}
%     0 \leq d(x,x) \leq \int_0^1 \sqrt{0M(x)0} d\lambda_1 = 0
% \end{align}
% Moreover, we see that
% \begin{equation}
% \begin{aligned}
%     d(x,y) &= \inf_{\gamma\in \Gamma^f_{x,y}} \int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, d\lambda_1 \\ &\geq \inf_{\gamma \in \Gamma_{x,y}} \int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, d\lambda_1 \\ &\geq \sqrt{\epsilon}\inf_{\gamma\in \Gamma_{x,y}} \int_{0}^1 ||\gamma'(t)|| \, d\lambda_1 \geq \sqrt{\epsilon}||x-y||
% \end{aligned}
% \end{equation}
% where $\Gamma_{x,y}$ is the same as $\Gamma_{x,y}^f$ except that the condition that the curve has to avoid the measure zero set is removed. From this inequality, we see that $d(x,y) > 0$ for $x \neq y$. Next we show the symmetry. For any $\gamma \in \Gamma_{x,y}^f$, it is clear that the reverse curve $\tilde{\gamma}(t):= \gamma(1-t)$ is an element of $\Gamma_{y,x}^f$. By a change of variable we have
% \begin{equation}
%     \begin{aligned}
%         \int_0^1 \sqrt{\gamma'(t)^TM(\gamma(t))\gamma'(t)} \, dt &=  \int_0^1 \sqrt{\tilde{\gamma}(t)^TM(\tilde{\gamma}(t))\tilde{\gamma}'(t)} \, dt
%     \end{aligned}
% \end{equation}
% So as the action of taking reverse curve gives a bijection between $\Gamma^f_{x,y}$ and $\Gamma^f_{y,x}$, we must have $d(x,y) = d(y,x)$. Finally we show triangle inequality. For any $\gamma_1 \in \Gamma_{x,y}^f$ and $\gamma_2 \in \Gamma_{y,z}^f$, we concat $\gamma_1$ and $\gamma_2$ to build $\gamma_3$
% \begin{align}
%     \gamma_3(t) = \begin{cases}
%         \gamma_1(2t), \quad t \in [0,\frac{1}{2}] \\
%         \gamma_2(2t - 1), \quad t \in [\frac{1}{2}, 1]
%     \end{cases}
% \end{align}
% Clearly $\gamma_3$ is still piecewise smooth. And since we have $G_{\gamma_3} \subset G_{\gamma_1} \cup G_{\gamma_2}$ where $G_\gamma := \{t: \gamma(t) \in G\}$, clearly we have $\lambda_1(G_{\gamma_3}) = 0$ and therefore $\gamma_3 \in \Gamma_{x,z}^f$. Now by simple change of variable we have
% \begin{equation}
%     \begin{aligned}
%         \int_{0}^1 \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt &= \int_{0}^1 \sqrt{\gamma_1'(t)^TM(\gamma_1(t))\gamma_1'(t)} \, dt + \int_{0}^1 \sqrt{\gamma_2'(t)^TM(\gamma_2(t))\gamma_2'(t)} \, dt
%     \end{aligned}
% \end{equation}
% Now taking infimum over both side we will get $d(x,z) \leq d(x,y) + d(y,z)$. \hfill $\square$

% \bigskip
% \noindent
% \textbf{Proof of Thm~\ref{thm:main}} Now we are finally ready to show the implication from condition~\eqref{verification} to contraction under the metric~\eqref{metric}. For any $\gamma \in \Gamma_{x,y}^f$, we consider the curve $f(\gamma)$. As $\mathcal{X}$ is forward invariant, $f(\gamma)$ also belongs to $\mathcal{X}$. By the verification condition~\eqref{verification}, we know that for $\delta_t$ small enough we always have 
% \begin{equation}\label{condition1}
% \begin{aligned}
%     (f(\gamma(t+\delta_t)) &- f(\gamma(t)))^TM(f(\gamma(t+\delta_t)))(f(\gamma(t+\delta_t)) - f(\gamma(t))) \\ &\leq \rho^2 (\gamma(t+\delta_t)-\gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t)-\gamma(t))\\
%     &< \rho'^2 (\gamma(t+\delta_t)-\gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t)-\gamma(t))
% \end{aligned}
% \end{equation}
% for some $\rho' \in (\rho, 1)$. Now fix an $\epsilon > 0$, we know that $f(\gamma)$ is a continuous curve, so that we can construct a piecewise smooth curve $\gamma_p$ such that $||f(\gamma(t)) - \gamma_p(t)|| \leq \epsilon$ for any $t$. And by previous construction, we know that there exists $\delta > 0$ such that for any $||v|| < \delta$, almost all the piecewise smooth curve
% \begin{align}
%     \gamma_v(t) = \gamma_p(t) + \eta(t)\sum_{i}v_iN_i(t)
% \end{align}
% intersect $G$ only on a measure zero set with $N_i$ constructed using $\gamma_p$. Pick one specific $\gamma_v$ now, and we would have 
% \begin{align}
%     ||\gamma_v(t) - \gamma_p(t)|| \leq \delta|\eta(t)| \leq \delta
% \end{align}
% Now suppose that we pick $\delta$ small enough such that $\delta < \epsilon$. By triangle inequality, we have
% \begin{align}
%     ||\gamma_v(t) - f(\gamma(t))|| \leq ||\gamma_v(t) - \gamma_p(t)|| + ||\gamma_p(t) - f(\gamma(t))|| \leq 2\epsilon
% \end{align}
% for any $t$. Now we see that we have
% \begin{equation}
% \begin{aligned}
%     % |f(\gamma(t+\delta_t)) - f(\gamma(t))| &= f(\gamma(t+\delta_t)) - \gamma_v(t+\delta_t) + \gamma_v(t+\delta_t) - \gamma_v(t) + \gamma_v(t) -  f(\gamma(t)) \\ &\leq 4\epsilon + |\gamma_v(t + \delta_t) - \gamma_v(t)| \\
%      |(f(\gamma(t+\delta_t)) - f(\gamma(t))) &- (\gamma_v(t+\delta_t) - \gamma_v(t))| \\ &\leq |f(\gamma(t+\delta_t)) - \gamma_v(t+\delta_t)| + |f(\gamma(t)) - \gamma_v(t)| \leq 4\epsilon
% \end{aligned}
% \end{equation}
% Now by~\ref{condition1}, the inequality is strict when the contraction factor is $\rho'$. This gives us room to wiggle the curve $f(\gamma)$ to be $\gamma_v$, which clearly belongs to the set $\Gamma_{f(x),f(y)}^f$, when $\epsilon$ is chosen to be small enough as everything is continuous, and we shall have the inequality
% \begin{align}
%     (\gamma_v(t+\delta_t) - \gamma_v(t))^TM(\gamma_v(t+\delta_t)))(\gamma_v(t+\delta_t) - \gamma_v(t)) \\ \leq \rho'^2(\gamma(t+\delta_t) - \gamma(t))^TM(\gamma(t+\delta_t))(\gamma(t+\delta_t) - \gamma(t))
% \end{align}
% Now divide both side by $\delta_t^2$ and let it goes to zero, we get
% \begin{align}
%     \gamma_v'(t)^TM(\gamma_v(t))\gamma_v'(t) \leq \rho'^2\gamma'(t)^TM(\gamma(t))\gamma'(t)
% \end{align}
% almost everywhere except on those points where $\gamma$ or $\gamma_v$ are not differentiable. This then implies 
% \begin{align}
%     d(f(x),f(y)) &\leq \int_0^1 \sqrt{\gamma_v'(t)^TM(\gamma_v(t))\gamma_v'(t)} \, dt \\
%     &\leq \rho'\int_0^1 \sqrt{\gamma'(t)M(\gamma(t))\gamma'(t)} \, dt
% \end{align}
% Now taking infimum gives the desired contraction result.

% \begin{proof}
%     We first show that the defined $d(x,y)$ is a valid metric. 
%     \begin{enumerate}
%         \item \textbf{Positivity.} Clearly we have that $d(x,y) \geq 0$. And since $\Gamma_{x,x}$ only contains the constant function $x$, we have that 
%         \begin{align}
%             d(x,x) = \int_{0}^1 \sqrt{0^T M(x) 0} \, dt = 0.
%         \end{align}
%         Conversely, suppose that $d(x,y) = 0$, we must have $\sqrt{\gamma'(t)^TM(\gamma(t))\gamma(t)} = 0$ for any $\gamma \in \Gamma_{x,y}$. Since $M(x)$ is positive definite, this implies that $\gamma'(t) = 0$ and $\gamma$ is constant. So clearly $x = y$.
%         \item \textbf{Symmetricity.} For any curve $\gamma \in \Gamma_{x,y}$, we consider the reverse curve $\tilde{\gamma}(s) = \gamma(1-t)$. We can easily compute that
%         \begin{equation}
%             \begin{aligned}
%                 \int_{0}^1 \sqrt{\tilde{\gamma}'(t)^TM(\tilde{\gamma}(t))\tilde{\gamma}(t)}\, dt &= \int_{0}^1 \sqrt{\gamma'(1-t)^TM(\gamma(1-t))\gamma'(1-t)} \, dt \\
%                 &= \int_{0}^1 \sqrt{\gamma'(s)^TM(\gamma(s))\gamma'(s)} \, ds
%             \end{aligned}
%         \end{equation}
%         by a change of variable $s = 1 - t$. As the map of taking the reverse curve is a bijection between $\Gamma_{x,y}$ and $\Gamma_{y,x}$, clearly we have $d(x,y) = d(y,x)$.
%         \item \textbf{Triangle Inequality.} For two curves $\gamma_1$ connecting $x,y$ and $\gamma_2$ connecting $y,z$, we can build a new curve by concatenating $\gamma_1$ and $\gamma_2$. Formally, we construct $\gamma_3$ as
%         \begin{align}
%             \gamma_3 &= \begin{cases}
%                 \gamma_1(2t),  \quad t \in [0, \frac{1}{2}] \\
%                 \gamma_2(2t - 1), \quad t \in [\frac{1}{2}, 1]
%             \end{cases}
%         \end{align}
%         Now we can can compute that
%         \begin{equation}
%             \begin{aligned}
%                 \int_{0}^1 \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt &= \int_{0}^{\frac{1}{2}} \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt + \int_{\frac{1}{2}}^1 \sqrt{\gamma_3'(t)^TM(\gamma_3(t))\gamma_3'(t)} \, dt \\
%                 &= \int_{0}^1 \sqrt{\gamma_1'(t)^TM(\gamma_1(t))\gamma_1'(t) \, dt} + \int_{0}^1 \sqrt{\gamma_2'(t)^TM(\gamma_2(t))\gamma_2'(t) \, dt}
%             \end{aligned}
%         \end{equation}
%         Now taking infimum on the LHS, it is clear that we have
%         \begin{align}
%             d(x,z) &\leq \int_{0}^1 \sqrt{\gamma_1'(t)^TM(\gamma_1(t))\gamma_1'(t) \, dt} + \int_{0}^1 \sqrt{\gamma_2'(t)^TM(\gamma_2(t))\gamma_2'(t) \, dt}
%         \end{align}
%         Since this works for any $\gamma_1 \in \Gamma_{x,y}$ and any $\gamma_2 \in \Gamma_{y,z}$, we can take infimum over them on the RHS without affecting the inequality, effectively resulting in
%         \begin{align}
%             d(x,z) \leq d(x,y) + d(y,z)
%         \end{align}
%     \end{enumerate}
%     Now we are ready to prove that $f$ is contracting under this metric. For any $\gamma \in \Gamma_{x,y}$, it is clear that $f(\gamma) \in \Gamma_{f(x),f(y)}$ as $\mathcal{X}$ is forward invariant. Utilizing the condition we have, we know that for small enough $\delta_t$, we have
%     \begin{align}
%         \sqrt{(f(\gamma(t + \delta_t)) - f(\gamma(t)))^T M(f(\gamma(t+\delta_t)))(f(\gamma(t + \delta_t)) - f(\gamma(t)))} \\ \leq k\sqrt{(\gamma(t+\delta_t)-\gamma(t))^TM(\gamma(t + \delta_t)(\gamma(t+\delta_t) - \gamma(t))}
%     \end{align}
%     Now we divide $\delta_t^4$ both side and let $\delta_t$ goes to 0. This recovers that
%     \begin{align}
%     \sqrt{f'(\gamma(t))^TM(f(\gamma(t)))f'(\gamma(t))^T} \leq k\sqrt{\gamma'(t)^TM(\gamma(t))\gamma(t)}
%     \end{align}
%     Therefore, we see that
%     \begin{align}
%         d(f(x),f(y)) &\leq \int_{0}^1 \sqrt{f'(\gamma(t))^TM(f(\gamma(t)))f'(\gamma(t))^T} \, dt\\
%         &\leq k\int_0^1 \sqrt{\gamma'(t)^TM(\gamma(t))\gamma(t)} \, dt
%     \end{align}
%     Now we take infimum over the right hand side yields the desired contraction
%     \begin{align}
%         d(f(x),f(y)) \leq kd(x,y)
%     \end{align}
% \end{proof}

% \begin{theorem}
%     Suppose the learned metric $M(x)$ admits uniform lower and upper bound
%     \begin{align}
%         \epsilon I \leq M(x) \leq \mu I
%     \end{align}
%     then the dynamics $f$ is incrementally stable in the Euclidean metric. 
% \end{theorem}
